GKNet: grasp keypoint network for grasp candidates detection

Contemporary grasp detection approaches employ deep learning to achieve robustness to sensor and object model uncertainty. The two dominant approaches design either grasp-quality scoring or anchor-based grasp recognition networks. This paper presents a different approach to grasp detection by treating it as keypoint detection in image-space. The deep network detects each grasp candidate as a pair of keypoints, convertible to the grasp representationg = {x, y, w, {\theta}} T , rather than a triplet or quartet of corner points. Decreasing the detection difficulty by grouping keypoints into pairs boosts performance. To promote capturing dependencies between keypoints, a non-local module is incorporated into the network design. A final filtering strategy based on discrete and continuous orientation prediction removes false correspondences and further improves grasp detection performance. GKNet, the approach presented here, achieves a good balance between accuracy and speed on the Cornell and the abridged Jacquard datasets (96.9% and 98.39% at 41.67 and 23.26 fps). Follow-up experiments on a manipulator evaluate GKNet using 4 types of grasping experiments reflecting different nuisance sources: static grasping, dynamic grasping, grasping at varied camera angles, and bin picking. GKNet outperforms reference baselines in static and dynamic grasping experiments while showing robustness to varied camera viewpoints and moderate clutter. The results confirm the hypothesis that grasp keypoints are an effective output representation for deep grasp networks that provide robustness to expected nuisance factors.

==> discussion.tex <==
\section{Discussion}
\subsection{Classification v.s. Regression}
One of the major differences between this work and previous approaches is to classify grasp angles into different categories, rather than directly regress to a single angle. This trick is based on the fact that CNNs are known to perform better classification task than regression task. Our experiments also shows that classification results indeed reflects the orientation of grasp, whereas the regressed angles tend to be erroneous. One drawback of regression based approach is that, the output usually regresses to the center of potential grasp due to averaging effect as in Fig. \ref{fig_case_not_averaged}. Also, regressed location is easily off the desired grasp. Fig. \ref{fig_case_failure_original} shows some failure cases of regression based approach. One other benefit of doing classification on candidate regions is that we can thus avoid manipulating rotated feature maps between network layers, which may potentially cause error due to the size of feature maps is typically small close to the output.  



\subsection{What objects are missing?}
One can observe that although we achieve high precision rate, the recall rate shows that we are unable to detect grasps one some objects. Before we investigate further, note that regression based approach always produces a predicted region, while our approach only predict one or more grasps when the system is confidential. Hence, the recall rate for previous approach is 100\% whereas ours is lower. Now, once a candidate region is produced by our system, we require the highest softmax score among all classes is above the threshold(0.8 in this work). And the system assigns class label representing the orientation of grasp to the candidate region. This might cause problem in two cases. The first case is when the object is round shape. And the second case is when the object is too small in the input image. Two cases cause the system find it hard to decide which orientation to assign, and the softmax scores for each class are equally small and below threshold. We output the images with missing grasp in Fig. \ref{fig_case_not_detected}. and it confirms our guess.















%\begin{figure}[t]
%    \centering
%    \includegraphics[width=2.8in]{fig_case_failure_original}
%    \caption{Failure cases of \cite{redmon2015real}. Regression tends to shift %from objects and causes invalid predictions.}
%    \label{fig_case_failure_original}
%\end{figure}

  

\begin{figure}[t]
    \centering
    \includegraphics[width=3.4in]{fig_case_not_detected}
    \caption{Failure cases using classification instead of regression. Round-shape like objects and tiny objects may have similar scores across all types of grasp, resulting in none of them has score above threshold, and thus no predicted grasps.}
    \label{fig_case_not_detected}
\end{figure}





\subsection{Multiple Grasps}
Our work is able to predict multiple grasp candidates without using sliding windows or dividing original input image into several grid. Hence the processing time is fast and the position of possible grasps is not limited to the grid cell. With more high quality grasps predicted, this system provides options for users to select most appropriate grasp to manipulate object. For example, one can choose the closest grasp, or choose grasp based on the functionality or the purpose of robot.      


\subsection{Pre-trained networks}
We chose to replace one of the original RGB channel with depth data in order to re-use pre-trained weights. A good pre-trained network is greatly helpful to quickly converge to better local minima point other than stuck in bad local minima. In our case the pre-trained weights originally for RGB seem to also work nicely for RGD data. By using VGG trained on ImageNet, this architecture is able to learn meaningful region proposal, regression and classification. Multiple grasp candidates can be predicted for novel objects.    




==> experiment.tex <==
The Grasp Keypoint Network approach to grasp recognition is a visual
processing approach intended to integrate with a robotic
manipulation pipeline. Consequently, evaluation of the approach will
involve both benchmarking as a visual input/output method, and as a
component in a larger manipulation process with an actual manipulator.
%
Visual processing will consider the accuracy of the output and the
timing of the method relative to other published one-stage, two-stage,
grasp quality and other deep learning approaches \citep{jiang2011efficient, 
asif2017rgb, lenz2015deep, mahler2017dex, morrison2019learning, wang2016robot, 
redmon2015real, kumra2017robotic, guo2017hybrid, zhou2018fully, chu2018real, 
asif2019densely}.

Manipulation experiments will include several different test and evaluation
methods found in the literature, or intended to demonstrate functional
characteristics. They are:
(1) static grasping, 
(2) dynamic grasping, and 
(3) grasping at varied camera angles and 
(4) bin picking. 
Static grasping is a simple test requiring precise grasp detection for
isolated objects, and is commonly performed to establish upper bounds on
performance due to the lack of distractors and impediments to grasping.
%
Dynamic grasping experiments test the combination of accuracy and speed,
but require some additional outer-loop elements for converting the grasp
detection system into a grasp tracking one. The experiments primarily
test for speed, with the resulting accuracy gap relative to static
grasping also being an indication of grasp detection consistency.
%
Grasping under varied camera angles tests the robustness with respect to
viewpoint and demonstrates some form of generalization of the algorithm
relative to this factor.
%
The bin picking experiment is the most challenging of the four since
grasp detection pipelines require additional outer-loop and
post-processing elements to identify a preferred grasp. Unlike grasp
quality networks, which can be trained under these circumstances,
one-stage and two-stage detectors are usually not trained to work in
these settings.
Some grasp quality networks benefit from simulation for amassing very
large ground-truth data, which can be several orders of magnitude larger
than for manually annotated datasets 
%\textcolor{purple}{Why this part is marked as red? I've confirmed that dataset proposed by dex-net has approximately 6.7 million datapoints while the Cornell dataset has 1035 images.}
{(i.e., DexNet grasp data is three
orders of magnitude more than the Cornell benchmark dataset).}
Conducting this experiment will involve introducing a simple grasp
prioritization scheme through a model-based grasp scoring system. 
%much like the score a grasp quality network is trained to output.

Prior to discussing the outcomes of the various experiments, this
section describes the GKNet training process, the experimental
evaluation criteria, and any additional common methodological elements
associated to the different experiments. Included in the latter is a
discussion about the test object sets. %protocols and evaluation metrics. 

\subsection{Datasets and Preprocessing \label{secDataTrain}}

There are two benchmark datasets commonly used for training and testing
grasp detection networks: the Cornell and Jacquard datasets 
\citep{cornell2013,depierre2018jacquard}.
The Cornell dataset contains 885 RGB-D images of 244 different objects,
with multiple images taken of each object from different poses. The
image dataset was collected and manually annotated with 5,110 positive
and 2,909 negative grasps. Though the Cornell dataset is used as a
standard dataset, annotation is relatively sparse and its size
is small. 
%
Based on a subset of ShapeNet \citep{chang2015shapenet}, the
simulation-based Jacquard dataset has more than 50,000 images of
11,000 objects, with 1 million {\em positive} grasps.  

\subsubsection{Cornell Dataset.}
Following other RGB-D implementations already trained on pre-existing
backbones for a different task (e.g., object
detection), we pass to the network the RG-D channels only by using the
depth channel as the blue channel input \citep{redmon2015real}. 
The depth information is normalized to lie in the same range, $[0,255]$,
as the RGB data.  All input channels are re-scaled to lie in the range
$[0,1]$, followed by a whitening process (per channel, per pixel, mean
value subtraction with division by the standard deviation).  The
obtained mean values for the RG-D channels are (0.85, 0.81, 0.25), with
standard deviations of (0.10, 0.11, 0.09).
%
The image resolution and annotation coordinates are remapped to the
matrix dimensions 227$\times$227, followed by application of the data
augmentation strategy presented in \citep{chu2018real} to increase the
amount of annotated input/output data and avoid model overfitting.


\subsubsection{Jacquard Dataset.}
The annotations in the Jacquard dataset were automatically generated in
order to have a much larger training set relative to the Cornell dataset
without the manual annotation demands.  Done in simulation, the grasps
were obtained via a sample and confirm process.
Compared with the Cornell dataset, images in the Jacquard dataset are
annotated with much denser grasping bounding boxes, however they are not
all physically meaningful. 
While the Cornell dataset has many missing (false negative) annotations,
the Jacquard dataset has several false positive annotations as well as
missing annotations.
After reviewing the dataset, we identified the following four problems
with the annotations:
%
(1) They can be dense on one side but sparse or even missing on the other
  side for some objects with symmetric shapes, 
  see Fig.  \sfigref{fig_jac_fail_case}a; 
%
(2) Some do not seem plausible and may be a function of incorrect
  physics within the simulator, see Fig. \sfigref{fig_jac_fail_case}b; 
%
(3) The sampling process can lead to sparse annotations for certain
  objects with multiple, continuous grasp regions, see
  Fig. \sfigref{fig_jac_fail_case}c, 
%
(4) Orientation dependent grasp annotations lead to highly variable
grasp annotation outcomes for the same object, Fig.
\sfigref{fig_jac_fail_case}d. 
%(1) The annotations can be dense on the one side but sparse or even missing on the other side for some objects with symmetric shapes like square. 
%%
%(2) The annotations of some objects are completely unreasonable. 
%%
%(3) The annotation is overall sparse relative to some certain objects with too many potential grasp candidates. 
%%
%(4) For the images of the same object with different poses, the distribution of grasp annotation can vary significantly. 
%%
%Visualization sample is provided for images with these four problems in Fig. \ref{fig_jac_fail_case}. 
%
These issues negatively influence the training process and the test evaluation
processes. 
%and they negatively influence the test evaluation criteria.

To correct for these issues, we defined a filtering strategy for
selecting a subset from the Jacquard dataset.
%
The filter strategy follows three rules based on the ratio of the union
of all grasp regions to the masked region of the object: 
%
(a) Keep annotation data whose ratio is larger than 0.8;
(b) Remove annotation data whose ratio is less than 0.2; and 
%
(c) Manually check images whose ratio is between 0.2 and 0.8 and remove
  those images whose annotations satisfy either one of the above four
  cases.
%
We call the resulting selected subset the Abridged Jacquard Dataset
(AJD), which is publicly available \citep{AJD}. The AJD consists of 
46{,}857 images of 10{,}799 objects, with 4{,}420{,}953 positive 
grasp bounding boxes in total. 

\begin{figure}[t]
  \centering
  \vspace*{0.05in}
  \begin{tikzpicture} [outer sep=0pt, inner sep=0pt]
  \scope[nodes={inner sep=0,outer sep=0}] 
  \node[anchor=north west] (a) at (0in,0in) 
    {\includegraphics[width=3cm,clip=true,trim=0in 0in 0in 0in]{fig_jac_fail_a.png}}; 
  \node[anchor=north west, yshift=-0.1cm] (b) at (a.south west) 
    {\includegraphics[width=3cm,clip=true,trim=0in 0in 0in 0in]{fig_jac_fail_b.png}}; 
  \node[anchor=north west, xshift=0.1cm] (c) at (a.north east) 
    {\includegraphics[width=4.53cm,clip=true,trim=0in 0in 0in 0in]{fig_jac_fail_c.png}};
  \node[anchor=north west, yshift=-0.1cm] (d) at (b.south west) 
    {\includegraphics[width=7.63cm,clip=true,trim=0in 0in 0in 0in]{fig_jac_fail_d.png}}; 
  \endscope
  \foreach \n in {a,b,c,d} { 
    \node[anchor=north west,xshift=2pt,yshift=-2pt] at (\n.north west) {(\n)};
  }
  \end{tikzpicture}
  \caption{
  (a)-(d): Four issues with the Jacquard dataset.
    \label{fig_jac_fail_case}}
  \vspace*{-1.0ex}
\end{figure}


%Due to downsampling of output keypoint heatmaps, multiple grasp keypoints on the input image can fall into the same pixel on the heatmap. This problem won't affect the prediction of heatmap but can be harmful to predictions of embedding and offset maps. For groundtruth of embedding map, there will be more than 2 keypoints have the same embedding value, which will leads to failure of grouping. For groundtruth of offset map, since one pixel on the offset map can only contain associated offsets for one grasp candidate, the problem will leads to inaccuracy to other grasp candidates whose ones of grasp keypoints fall into that pixel on the offset map. To deal with this problem, we filter the dense annotation out to make sure that there will not be any points from different grasp bounding boxes fall into the same pixel on the downsampled map. 
Due to downsampling of output keypoint heatmaps relative to the input
image, multiple grasp keypoints from different grasp instances can map
to the same pixel in the ground truth heatmap.
%
For example, if the left-middle point of grasp instance $A$ is within
the radius of downsampling ratio of the left-middle point of grasp
instance $B$ on the input image, they will be located at the same pixel
on the groundtruth heatmap. 
%
To deal with the resulting ambiguity, we refine the dense annotations 
by always selecting the first grasp bounding box processed
to make sure that there will not be any points from different grasp
bounding boxes mapping to the same pixel on the downsampled map.
%
The above strategy isn't applied to the Cornell dataset, since its
grasp annotations are sparse. 

%
Image normalization follows the same procedure applied to the Cornell
dataset. The mean values of the RG-D channels are (0.71, 0.71, 0.20),
and the standard deviations are (0.06, 0.07, 0.09).  The Jacquard images
and annotations were remapped to the matrix dimensions 512$\times$512,
with no data augmentation applied. 

\subsection{Deep Network Architecture and Training}

We use Deep Layer Aggregation (DLA) as our backbone network to extract
features from input images \cite{yu2018deep}.  DLA augments standard
neural network architectures with an iterative and hierarchical aggregation strategy to fuse semantic and spatial information across layers. The deep layer aggregation structures helps network capture deeper and wider information for recognition and localization. Meanwhile the hierarchy aggregation architecture requires fewer parameters, which reduces size of the entire network and inference time. 
We choose DLA as our final backbone network since it achieves the best
performance. Rich semantic and spatial information improves performance
of keypoint detection and fewer network parameters enables GKNet to run
in real-time. However there is no restriction on the backbone network
for GKNet; it can be switched to other state-of-the-art keypoint
detection neural networks. 
%

%Additionally, we incorporate a non-local module based on fact that two grasp keypoints have strong dependency between each other. Non-local operation is a simple but efficient module in computer vision for capturing long-range dependencies with deep neural networks. As shown in Fig. \ref{fig_netarch}, we insert it between backbone network and grasp hypothesis branch to help learn dependencies with associated embedding maps of \emph{grasp keypoint heatmaps}.

Our work is implemented in PyTorch \cite{paszke2017automatic} and the backbone network DLA is pretrained on ImageNet \cite{deng2009imagenet}. 
We use random affine transformation as data augmentation and use Adam \cite{diederik2015adam} to optimize training loss:
\begin{align} \label{training_loss}
  \loss{}{} = \loss{det}{gk} + \loss{det}{aux} 
                + \alpha \loss{pull}{gk} + \beta \loss{push}{gk} 
                + \gamma \loss{off}{gk},
\end{align}
where $\alpha$, $\beta$ and $\gamma$ are the weights of the pull, push
and offset loss for \emph{grasp keypoint heatmap}. 
For training, we use a batch size of 8 and train our network end-to-end
on a single Titan XP. 
%
For the Cornell dataset, we train for 20 epochs with the initial
learning rate of $1.25 \times 10^{-4}$ and divided by 10 at the 10th and
the 15th epoch. 
%
For the AJD, we train for 30 epochs with the same initial learning rate
and with divisions at the 20th and the 25th epoch.

\begin{figure*}[t]
  \centering
  \scalebox{0.98}{
  \begin{tikzpicture} [outer sep=0pt, inner sep=0pt]
  \scope[nodes={inner sep=0,outer sep=0}] 
  \node[anchor=north west] (a) at (0in,0in) 
    {\includegraphics[width=4.35cm,clip=true,trim=0in 0.0in 0in 0in]{fig_hh_set1.jpg}}; 
  \node[anchor=north west, yshift=-0.1cm] (b) at (a.south west)
    {{\includegraphics[width=4.35cm,clip=true,trim=0in 0.0in 0in 0in]{fig_hh_set2.jpg}}}; 
  \node[anchor=north west, xshift=0.1cm] (c) at (a.north east)
    {\includegraphics[width=3.95cm,clip=true,trim=0.0in 0.0in 0.0in 0.0in]{fig_ad_set.jpg}}; 
    \node[anchor=north west, xshift=0.1cm, yshift=-0.1cm] (d) at (a.south east)
    {\includegraphics[width=3.95cm,clip=true,trim=0.0in 0.0in 0.0in 0.0in]{fig_mix_set.jpg}}; 
    %\node[anchor=north west, yshift=-0.1cm] (e) at (b.south west)
    \node[anchor=north west, xshift=0.1cm] (e) at (c.north east)
    {\includegraphics[width=8.9cm,clip=true,trim=0.0in 0.0in 0.0in 0.0in]{fig_bp_set.jpg}}; 
  \endscope

  \foreach \n in {a,b,c,d,e} 
   {
    \node[anchor=north west,fill=white,draw=white,inner sep=1pt] at (\n.north west) {(\n)};
   }
  \end{tikzpicture}}
  \vspace*{-0.25ex}
  \caption{
    Object sets used for two grasp experiments. (a) The household set (Morrison). (b) The household set (Chu). (c) The adversarial set. (d) The compound set. (e) The bin picking object set.
    \label{fig_obj_set}}
\end{figure*}


\subsection{Parameters}

We report some essential hyper-parameters used in training and testing
process here; the rest are available in the released code \citep{ivagit_GKNet}. 
With a downsampling ratio of $\redFact = 4$, GKNet outputs heatmaps with
size of 57$\times$57 and 128$\times$128, for the Cornell and Jacquard
dataset respectively. 
For all training processes, we choose weighting coefficients in
(\ref{training_loss}) to be $\alpha = 1$, $\beta = 1$ and $\gamma = 1$.
Due to the different image source and grasp annotation distributions,
we set different testing stage filtering coefficients 
$\threshEmbed$, $\threshCenter$ and $\threshOrient$ for the 
datasets.

\vspace*{0.25em}
\noindent
\textbf{Cornell.}
We set 
$\threshEmbed = 1.0$, 
$\threshCenter = 0.05$ and 
$\threshOrient = 0.24$. 
The number of orientation classes is $\left| \oclass \right| = 18$.

\vspace*{0.25em}
\noindent
\textbf{AJD.}
We set 
$\threshEmbed=0.65$, 
$\threshCenter=0.15$, and 
$\threshOrient=0.1745$. 
The number of orientation classes is $\left| \oclass \right| = 36$.

\subsection{Evaluation Metrics for Vision Benchmarking}
The standard grasp evaluation metric considers the full grasp rectangle
\citep{redmon2015real}.  By design, the GKNet grasp representation
lacks the variable $h$ describing the bounding box. To apply the same
evaluation metric as other publications, the value $h$ is set to the
average of all grasp candidates for the training dataset used.  These
values work out to be 23.33 and 20 for the Cornell dataset and the AJD,
respectively.  The predicted grasp candidate is a positive match if:
\begin{enumerate}
  \item the orientation difference between predicted grasp and
  corresponding ground truth is within 30$^\circ$; and 
  \item the Jaccard index of the predicted grasp $g_p$ and the ground truth grasp $g_t$ is greater than 0.25:
    \begin{equation} \label{eqn_jaccard_index}
      J(g_p,g_t) = \frac{\vert g_p \cap g_t \vert}{\vert g_p \cup g_t \vert} 
                 > \frac 14.
    \end{equation}
\end{enumerate}
The speed of the grasp recognition process is measured in frames per
second (fps).

\subsection{Objects Sets for Manipulation Experiments}

Though there are published robotic benchmark object datasets like
the ACRV Picking Benchmark (APB)
and the YCB Object Set  \citep{calli2015benchmarking,leitner2017acrv},
most published works employ their own objects or a subset of objects
from these datasets.  For comparison purposes, we employ 5 object sets
for 4 different kinds of robotic grasping experiments. 
The test sets include novel objects not included in the training datasets. 
They are described below and visualized in Fig. \refsp{fig_obj_set}.
They have some overlap with the APB and YCB sets.

\vspace*{0.25em}
\noindent
{\bf Household Sets.} 
The two different household sets are shown in Fig. \sfigref{fig_obj_set}a 
and \sfigref{fig_obj_set}b, 
as described in \cite{morrison2019learning} and \cite{chu2018real}.
The Morrison set contains 12 common household objects of different sizes
and shapes. The objects were chosen from the standard robotic grasping
datasets \citep{calli2015benchmarking,leitner2017acrv}.
The Chu set contains ten commonly seen objects collected from the
Cornell dataset.

\noindent
{\bf Adversarial Set.} 
The adversarial set, shown in Fig. \sfigref{fig_obj_set}c, consists of eight
3D-printed objects described in Dex-Net 2.0 \citep{mahler2017dex}. 
The objects are characterised by complex and adversarial geometric
features such as smooth and curved surfaces, which increase the
difficulty of grasping. They are meant to undermine grasp scoring
systems. It is less clear what impact these shapes have on other
learning-based grasping approaches.

\noindent
{\bf Compound Set.} The compound set, shown in Fig. \sfigref{fig_obj_set}d,
is composed of seven common household objects and 3 objects from the
adversarial set.

\noindent
{\bf Bin Picking Object Set.} 
The bin picking object set, shown in Fig. \sfigref{fig_obj_set}e, is
collected for bin picking experiments. The object set has 50 objects
consisting of household objects and adversarial objects.

\subsection{Evaluation Metrics for Manipulation Experiments}

Unless otherwise stated, the evaluation criteria for the grasping
experiments will consist of the grasping success rate, which is the
percentage of successful grasps relative to the total amount of grasp
attempts.  A grasp is considered to be a success if the manipulator
grasps, lifts, and holds object in the air for three seconds.
While some researchers also measure--and advocate for--
{\em mean picks per hour} \citep{mahler2016dex}, we elect to not include this
quantitative measure as it is influenced more by the manipulator
properties, the manipulation code, and the programmed grasping
procedure, than by the visual processing algorithm. In short, within the
perception, planning, and action loop, the planning and action steps
determine the pick rate more so than the perception step. 
This manuscript's scope is related to the perception process, not to the
planning and action processes.

\subsection{Trained Models for Manipulation Experiments}
For the majority of the manipulation experiments, 
the Cornell dataset was the training dataset.  This permits evaluation of 
approaches that trained and tested against Cornell, and also performed
manipulation experiments. Some methods have a performance gap when moving 
from visual processing to embodied grasping, which train and test data 
consistency permits comparing with.
The one exception is for the bin picking experiment, where GKNet was
trained with the AJD.  Bin picking scenarios involve multiple objects,
for which neither the AJD nor the Cornell dataset has the equivalent
type of training data; both consist of scenes with a single object only.  
The choice to use AJD is due to differences in the annotation sparsity,
or in the ground-truth grasp distributions, between the Cornell dataset
and the AJD.  The denser annotations in the AJD dataset better aid in
locating grasps for object sub-parts, whereas models trained on the
Cornell dataset  tend to provide grasp candidates with respect to the
whole object.  For cluttered environments with overlaid or occluded
objects, the ability to focus on sub-parts improves the ability to
differentiate occlusion geometries and target object regions.


